Offline Trace Checking of Quantitative Properties of Service-Based Applications

Service-based applications are often developed as compositions of partner services. A service integrator needs precise methods to specify the quality attributes expected by each partner service, as well as effective techniques to verify these attributes. In previous work, we identified the most common specification patterns related to provisioning service-based applications and developed an expressive specification language (SOLOIST) that supports them. SOLOIST is an extension of metric temporal logic with aggregate temporal modalities that can be used to write quantitative temporal properties. In this paper we address the problem of performing offline checking of service execution traces against quantitative requirements specifications written in SOLOIST. We present a translation of SOLOIST into CLTLB(D), a variant of linear temporal logic, and reduce the trace checking of SOLOIST to bounded satisfiability checking of CLTLB(D), which is supported by ZOT, an SMT-based verification toolkit. We detail the results of applying the proposed offline trace checking procedure to different types of traces, and compare its performance with previous work.

==> encoding.tex <==

\section{Optimized Translation}
\label{sec:optim-transl}

The major drawback of the basic translation is the size of the
resulting MPLTL formula, which impacts on the efficiency of the
verification; this is mainly due to the way the $\mathfrak{C}$ and
$\mathfrak{D}$ modalities are translated.
In this section we propose a
 more succinct and efficient translation  for 
these two modalities. The new, optimized translation is based on 
CLTLB($\mathcal{D}$)~\cite{bersani12:_const_ltl_satis_check_autom},
an extension of  PLTLB (Propositional Linear Temporal Logic with both past
and future modalities) augmented with atomic formulae built over a
constraint system $\mathcal{D}$. In practice, CLTLB($\mathcal{D}$)
supports the definition of 
\emph{counter variables} and \emph{arithmetical constraints} over a constraint
system $\mathcal{D}$; in our case $\mathcal{D}$ 
is the structure $(\mathbb{Z},<)$, for which decidability has been
proven in~\cite{demri07:_ltl}.
Counter variables (or \emph{counters}) are variables that receive a separate evaluation at
each time instant. In addition to the standard PLTLB syntax,
CLTLB($\mathcal{D}$) introduces the new construct of \emph{arithmetic
temporal term}, defined as $\alpha := c \mid x \mid \mathsf{Y}(x) \mid
\mathsf{X}(x)$, where $c$ is a constant, $x$ is a counter and $\mathsf{Y}$ and
$\mathsf{X}$ are temporal operators applied to counters that, unlike their
PLTLB counterparts, return the value of the counter in the previous
and in the next time instant, respectively. In CLTLB($\mathcal{D}$)
atomic formulae can also be formulae of the form 
 $\mathit{R}(\alpha_1, \alpha_2, \ldots, \alpha_n)$, where
$\mathit{R}$ is an arithmetical constraint.
Since  CLTLB($\mathcal{D}$) is an extension of PLTLB, we can define  all constructs
of MPLTL through it. As done for the basic translation, here we also
assume that \sol formulae are single-sorted,
quantifier-free and in normal form, with their semantics defined over
$\omega$-words.

Before presenting  the optimized translation, we introduce some useful notations.
Events can occur multiple times in a history trace;  when we refer to a specific occurrence of an event $\phi$ at a time instant $\tau$, we denote this as $\phi_{|\tau}$.
Let $x$ and $y$ be finite counters modulo $K+1$, then for $K' \leq K$
we define the following two macros:
%\begin{small}
\begin{compactitem}
\item $W(K, K^\prime,x, y) = $  \texttt{if} $(\mathsf{X}(x) - \mathsf{Y}^{K^\prime-1}(y) \geq
0)$ \\ \texttt{then} $\mathsf{X}(x) - Y^{K^\prime-1}(y)$ \texttt{else} $\mathsf{X}(x) - Y^{K^\prime-1}(y) + (K+1)$ 
\item $W1(K, K^\prime, x) = W(K, K^\prime, x, x)$ 
\end{compactitem}
%\end{small}



The $W(K, K^\prime,x, y)$ macro returns the difference between the values of the counters 
$x$ and $y$, but considered at different time instants. 
With respect to the time instant where the macro is evaluated, the 
value of $x$ is taken at the 
next time instant, while the value of $y$ is taken $K^\prime-1$ time instants in the past. 
Consider, for example, Fig.~\ref{fig:macro}.
If the macro $W(9,4,x,y)$ is evaluated at time instant $\tau$, it will
return 7, which is the difference between 9, the value of $x$ at time
instant $\tau+1$, and 2, the value of $y$ at time
instant $\tau-(K^\prime - 1)=\tau-3$; the values of the counters
considered for the evaluation of the macro are circled in the picture.
 If the difference between the values is less then zero, the macro adds to the result 
the modulo  of the counters. 
% Consider now Fig.~\ref{fig:WmacroMod}. The macro 
% $W(9,4,x,y)$, when evaluated  at $\tau$,  returns  9,  which is obtained
% by adding the modulo of the counters ($K+1=10$) to the difference
% between 6, the value of $x$ at time
% instant $\tau+1$,  and 7, the value of $y$ at time
% instant $\tau-(K^\prime - 1)=\tau-3$.
The macro $W1$ applies the macro $W$ to the same counter.

% Using these macros we can relate a counter to an event and express
% its number occurrences within a time window smaller than the modulo
% of the counter, under the assumption that it can't occur more than
% once per time instant.

\begin{figure}[!tbd]
        \centering
        % \subfloat[]{
        %     \begin{minipage}{\linewidth}
        % \centering
		\input{figures/wmacro}
            % \end{minipage}
	%\label{fig:Wmacro}
	% } 

        % \subfloat[]{
        %     \begin{minipage}{\linewidth}
        % \centering
	% 	\input{figures/wmacromod}
        %     \end{minipage}
	% \label{fig:WmacroMod}
	% } 
\caption{Evaluation of the macro $W$}
\label{fig:macro}
\end{figure}
In the rest of this section, we present the optimized translation for the  $\mathfrak{C}$ and $\mathfrak{D}$ modalities.

\subsection{Translation of the $\mathfrak{C}$ modality}
The $\mathfrak{C}$ modality expresses a bound on the number of
occurrences of a certain event in a given time window; it comes
natural to use the counters available in CLTLB($\mathcal{D}$) for the translation. 
Indeed, to translate a \sol formula containing sub-formulae with the
$\mathfrak{C}$ modality, we use a counter for the argument of each 
$\mathfrak{C}$ modality sub-formula. All counters are bounded by the value of
the largest time window that is referenced in any of the  $\mathfrak{C}$
modality sub-formulae; this value is denoted $K_{max}$.


For each sub-formula of the form $\mathfrak{C}_{\bowtie n}^K (\phi)$, we introduce a
finite counter  $c_{\phi} : 0 \ldots K_{max}$, constrained by the
following CLTLB($\mathcal{D}$) axioms:
\begin{compactenum}[{A}1)]
  \item \label{ca1} $c_\phi=0$
  \item \label{ca2} $\mathsf{G}((e \land \phi) \rightarrow \mathsf{X}(c_\phi)=(c_\phi+1)\mod{(K_{max}+1)})$
  \item \label{ca3}  $\mathsf{G}((\neg e \lor \neg \phi) \rightarrow \mathsf{X}(c_\phi)=c_\phi)$
\end{compactenum}


Axiom~A\ref{ca1} initializes the counter to zero. Axiom~A\ref{ca2} is
an implication: the antecedent corresponds to the occurrence of a
valid event $\phi$, denoted by the conjunction $e \land \phi$; in the
consequent, the value of the counter $c_\phi$ in the next time instant
is constrained to be increased by 1 with respect to the value at the
current time instant.  As it will be the case in the rest of this section, an increase of the value of the counters is always meant to
be done modulo $K_{max}+1$. Axiom~A\ref{ca3} refers to the opposite
situation, when either  there is no occurrence of the event $\phi$ or the time
instant is not valid. In this case,  the value of the
counter  in the next time instant is constrained to have the same
value as in the current time instant.
Both axioms~A\ref{ca2} and A\ref{ca3} have to hold at every time
instant, so they are in the scope of a   \textit{globally} 
modality.

A sub-formula of the form $\mathfrak{C}_{\bowtie n}^{K} (\phi)$ 
is then translated as $W1(K_{max},K,c_{\phi}) \bowtie n$.

Axioms~A\ref{ca1}, A\ref{ca2}, A\ref{ca3} constrain the behavior of
each counter $c_{\phi}$ so that  $c_{\phi}$ holds, at every time
instant $\tau$, the number of occurrences of event $\phi$ in the past.
Hence, we can calculate the exact number of occurrences by subtracting
the values of the counter at appropriate time instants, which is
exactly done by the macro $W1$.
The axioms are conjuncted with the resulting translation, thus
effectively constraining the behavior of the counters of the type $c_{\phi}$.

An example of the use of counters of the type $c_\phi$ is shown in
Fig.~\ref{fig:cmod}, which depicts a simple history trace and the
values assumed by the counter at each time instant, as determined by
the axioms. To evaluate the formula $\mathfrak{C}_{> 1}^{3}(\phi)$ at
time instant 13 against the sample trace, we first apply macro $W1$ to
subtract the value of the counter $c_\phi$ at time instant 11 from the
value at time instant 14 (values are marked with a circle). The
resulting value ($4-2=2$) is then compared to the specified bound.  If
we evaluate the formula $\mathfrak{C}_{> 1}^{5}(\phi)$ at time instant 8
of the same trace, we can see that the resulting value ($0-4+(5+1)=2$)
correctly reflects the number of events within the time window even in
the case when the difference between counters values is negative;
these values are marked with squares at time instants 9 and 4.

\begin{figure}
\centering
\input{figures/cmod}
\caption{Example of history trace for the $\mathfrak{C}$ modality}
\label{fig:cmod}
\end{figure}

\subsection{Translation of the $\mathfrak{D}$ modality }
The $\mathfrak{D}$ modality expresses a bound on the average distance
between the occurrences of pairs of events in a given time
window. For simplicity, we consider only (sub-)formulae of the $\mathfrak{D}$
modality that refer to one pair, like $\mathfrak{D}_{\bowtie n}^{K}\{(\phi, \psi)\}$.
%Before explaining the translation to CLTLB($\mathcal{D}$), we
%introduce some useful definitions. 

A pair of events $(\phi,\psi)$ may have multiple instances in a
history trace. We denote $(\phi_{|i},\psi_{|j})$ an instance, if there
is an occurrence of event $\phi$ at time instant $i$ and an occurrence
of event $\psi$ at time instant $j$, with $i<j$. We call such instance
\textit{open} at time instant $\tau$ if $i\leq\tau<j$.  Otherwise, the
instance is \textit{closed} at time instant $\tau$.
The \emph{distance} of a closed pair instance is $j-i$; for an open pair at time instant $\tau$, the distance is $\tau-i$.
 A time window
defined for a $\mathfrak{D}$ modality (sub-)formula evaluated at time
instant $\tau$ is bounded by the time instants $\tau+1$ and
$\tau-K+1$.  Given a history trace $H$, we say that a $\mathfrak{D}$
modality (sub-)formula for a pair of events $(\phi,\psi)$ has a
\textit{left-open} (respectively, \emph{right-open}) pair in $H$ if
there is an open instance of $(\phi,\psi)$ at time instant $\tau-K+1$
(respectively, $\tau+1$) in $H$.
Depending on whether a $\mathfrak{D}$ modality (sub-)formula contains
(left- and/or right-)open pairs or none, there are four distinct cases
to take into account for the translation.

For each sub-formula of the form  $\mathfrak{D}_{\bowtie n}^{K}\{(\phi,
\psi)\}$, we introduce
five counters. In the definition of the counters, $K_{max}$ is the
value of the largest time window that is referenced in any of the  $\mathfrak{D}$
modality sub-formulae. The counters are:
\begin{itemize}[-]
\item  $c_{\phi,\psi}: 0 \ldots 1$. This binary counter assumes value 1
  in the time instants following an occurrence of $\phi$ and is reset
  to 0 after an  occurrence of $\psi$. It acts as a flag denoting the
  time instants during which the event pair instance is open.
\item $h_{\phi,\psi}: 0 \ldots \lfloor\frac{K_{max}}{2}\rfloor$. Being increased
  after every occurrence of $\psi$,  in each time instant this counter
  contains the number of previously seen closed pair instances.
\item $s_{\phi,\psi}: 0 \ldots K_{max}$. It is increased at every time
  instant when either $c_{\phi,\psi}=1$ holds or  $\phi$ occurs. At each time instant, its
    value corresponds to  the sum of  distances of all previously
  occurred pair instances.
\item $a_{\phi,\psi}: 0 \ldots K_{max}$. It keeps track of the  sum of the  distances of all previously occurred closed pair instances.
\item $b_{\phi,\psi}: 0 \ldots K_{max}$. This counter has the values
  that will be assumed by counter  $s_{\phi,\psi}$  at the next occurrence of
  $\psi$ (more
  details below).
\end{itemize}
Counters $a_{\phi,\psi}$, $b_{\phi,\psi}$, and $h_{\phi,\psi}$ are used
directly in the translation of the $\mathfrak{D}$ modality (sub-)formulae, while
counters $c_{\phi,\psi}$ and $s_{\phi,\psi}$ are helper counters, used
to determine  the values of the other counters.

These counters are  constrained by the following  axioms:
\begin{compactenum}[{A}1)]
\setcounter{enumi}{3}
  \item \label{da4}  $c_{\phi,\psi}=0$ $\land$ $h_{\phi,\psi}=0$ $\land$ $a_{\phi,\psi}=0$ $\land$ $s_{\phi,\psi}=0$
  \item \label{da5} $(\mathsf{X}b_{\phi,\psi}=b_{\phi,\psi})\mathsf{W}(e \land \psi)$
  \item \label{da6} 
    \begin{tabbing}
 $\mathsf{G}$\=$((e \land \phi) \rightarrow (\mathsf{X}c_{\phi,\psi}=1 \land$ \\
\> $\mathsf{X}s_{\phi,\psi}=(s_{\phi,\psi}+1) \mod{(K_{max}+1)} \land$ \\
\> $\mathsf{X}h_{\phi,\psi}=h_{\phi,\psi} \land \mathsf{X}a_{\phi,\psi}=a_{\phi,\psi}))$ \\
\end{tabbing}
\vspace{-\baselineskip} 
  \item \label{da7}
    \begin{tabbing}
 $\mathsf{G}$\=$((e \land \psi) \rightarrow (\mathsf{X}c_{\phi,\psi}=0 \land$ \\
\> $\mathsf{X}h_{\phi,\psi}=(h_{\phi,\psi}+1)
\mod{(\lfloor\frac{K_{max}}{2}\rfloor+1)} \land$ \\
\> $\mathsf{X}a_{\phi,\psi}=s_{\phi,\psi} \land \mathsf{X}s_{\phi,\psi}=s_{\phi,\psi} \land b_{\phi,\psi}=s_{\phi,\psi}$ $\land$ \\
\> $\mathsf{X}((\mathsf{X}b_{\phi,\psi}=b_{\phi,\psi})\mathsf{W}(e \land \psi))))$  \\
\end{tabbing}
\vspace{-\baselineskip}
  \item \label{da8}
    \begin{tabbing}
 $\mathsf{G}$\=$((\neg e \lor (\neg \phi \land \neg \psi))
 \rightarrow (\mathsf{X}c_{\phi,\psi}=c_{\phi,\psi} \land$ \\
  \> $\mathsf{X}h_{\phi,\psi}=h_{\phi,\psi}$ $\land$ $\mathsf{X}a_{\phi,\psi}=a_{\phi,\psi}$ $\land$ \\
  \> $(c_{\phi,\psi}=1$ $\rightarrow$ $\mathsf{X}s_{\phi,\psi}=(s_{\phi,\psi}+1) \mod{(K_{max}+1)}) \land$ \\
  \> $(c_{\phi,\psi}=0$ $\rightarrow$ $\mathsf{X}s_{\phi,\psi}=s_{\phi,\psi}$))) \\
\end{tabbing}
\vspace{-\baselineskip}
  \end{compactenum}
 
  Axiom~A\ref{da4} initializes all counters except counter
  $b_{\phi,\psi}$, which will assume values determined by counter
  $s_{\phi,\psi}$.  Axiom~A\ref{da5} states that the value of counter
  $b_{\phi,\psi}$ will stay the same in all the consecutive time
  instants until the first occurrence of $\psi$. Notice that we use
  the $\mathsf{W}$ modality (``weak until''), to deal with traces
  without occurrences of $\psi$.  Axiom~A\ref{da6} determines the next
  time instant value of the following counters, upon occurrence of a
  $\phi$ event (denoted by $\phi \land e$): counter $c_{\phi,\psi}$ is
  set to 1; counter $s_{\phi,\psi}$ is incremented by 1; counters
  $h_{\phi,\psi}$ and $a_{\phi,\psi}$ are constrained not to change
  in the next time instant. Axiom~A\ref{da7} determines
  how the counters are updated when an event $\psi$ occurs: counter
  $c_{\phi,\psi}$ is set to 0; counters $b_{\phi,\psi}$,
  $\mathsf{X}a_{\phi,\psi}$, and $\mathsf{X}s_{\phi,\psi}$ are set to
  be equal to $s_{\phi,\psi}$. Moreover, axiom~A\ref{da5} is
  constrained to hold in the next time instant, forcing value of
  $b_{\phi,\psi}$ to stay the same in all the consecutive time
  instants until the next occurrence of $\psi$.  Axiom~A\ref{da8}
  covers the cases either when there are no valid events or when
  neither $\phi$ nor $\psi$ occur.  In these cases the values of
  counters $c_{\phi,\psi}$, $h_{\phi,\psi}$, and $a_{\phi,\psi}$ are
  constrained to stay the same, counter $b_{\phi,\psi}$ is
  unconstrained, while for $s_{\phi,\psi}$ we need to distinguish two
  separate cases.  When the pair instance is open (denoted by
  $c_{\phi,\psi}=1$), counter $s_{\phi,\psi}$ is incremented by 1,
  otherwise it stays the same.

  As said above, the $b_{\phi,\psi}$ counter keeps the values that
  will be assumed by counter $s_{\phi,\psi}$ at the next occurrence of
  $\psi$.  The value assumed by both counters $a_{\phi,\psi}$ and
  $b_{\phi,\psi}$ originates from counter $s_{\phi,\psi}$, as enforced
  by axiom~A\ref{da7}. Axioms~A\ref{da6} and A\ref{da8} make sure the
  value of $s_{\phi,\psi}$ is propagated in the future via counter
  $a_{\phi,\psi}$, while axioms~A\ref{da5} and A\ref{da7} enable the
  propagation of this value in the past via counter $b_{\phi,\psi}$.
  We elaborate this through an example: Fig.~\ref{fig:depend}
  represents a short history trace of length 11 with event $\psi$
  occurring at time instants 2 and 9.  The first row below the
  timeline denotes values of counter $s_{\phi,\psi}$ at different time
  instants, while the second row denotes the values of counter
  $b_{\phi,\psi}$.  Axiom~A\ref{da5} enforces equality (denoted with
  \tikz[baseline=-0.5ex]{ \draw[snake=zigzag,segment length=4pt] (0,0)
    -- (0.5,0); }) between successive values of counter
  $b_{\phi,\psi}$ at adjacent time instants until the first occurrence
  of $\psi$.  Additional equalities (of the same type) on the values
  of counter $b_{\phi,\psi}$ are enforced by axiom~A\ref{da7}. The
  same axiom also determines equality (denoted with
  \tikz[baseline=-0.5ex]{ \draw[snake=coil,segment length=4pt]
    (0,-0.25) -- (0,0.25); }) between the values of the
  $s_{\phi,\psi}$ and $b_{\phi,\psi}$ counters upon an occurrence of
  $\psi$.


\begin{figure}[tb]
\begin{center}
\input{figures/depend}
\end{center}
\caption{Propagation of the values of the counter  $b_{\phi,\psi}$}
\label{fig:depend}
\end{figure}


A sub-formula of the form $\mathfrak{D}_{\bowtie
  n}^{K}\{(\phi, \psi)\}$ is translated as:\\
\texttt{if}  ($\mathsf{Y}^{K-1}  (c_{\phi,\psi}) = 1$)\\
 \texttt{then} 
$\tfrac{W(K_{max},K,a_{\phi,\psi},b_{\phi,\psi})}{W1(\lfloor\frac{K_{max}}{2}\rfloor,
  K, h_{\phi,\psi})-1} \bowtie n$ \texttt{else} 
$\tfrac{W1(K_{max},K,a_{\phi,\psi})}{W1(\lfloor\frac{K_{max}}{2}\rfloor, K,
  h_{\phi,\psi})} \bowtie n $\\


The condition $\mathsf{Y}^{K} (c_{\phi,\psi}) = 1$ checks whether the
time window contains an open pair instance on its left bound. Notice
that semantics of the $\mathfrak{D}$ modality considers only closed
pairs within the time window to compute the average distance, so open
pairs are to be ignored both on the left and on the right bound of the
time window.  There is no need to differentiate between the cases
when there is a right-open pair, since counter $a_{\phi,\psi}$
only considers  distances between closed pair instances.
The numerator of the fraction in both the \texttt{then} and
\texttt{else} branches denotes the total
distance, while the denominator corresponds to the number of pair
instances considered for computing the total distance.
Axioms~A\ref{da4}, A\ref{da5}, A\ref{da6}, A\ref{da7}, A\ref{da8} are
conjuncted with the resulting translation and added as constraints
that hold at the initial time instant of the history trace.

An example of the use of counters for evaluating a formula with the $\mathfrak{D}$
modality is shown in Fig.~\ref{fig:dmod}, which depicts a simple history
trace and the values assumed by the counters  $c_{\phi,\psi}$,
$h_{\phi,\psi}$, $s_{\phi,\psi}$, $a_{\phi,\psi}$, and $b_{\phi,\psi}$
at each time instant, as
determined by the axioms. We notice that there are three 
instances of the  $(\phi, \psi)$ pair.
If we evaluate the formula
 $\mathfrak{D}_{\bowtie n}^{14}\{(\phi, \psi)\}$ at time instant 15  of
 the sample history trace, the two pair instances
 $(\phi_{|2},\psi_{|5})$ and $(\phi_{|9},\psi_{|14})$,  considered
 to compute the average distance, are closed. The left-hand side (lhs)
 of
 the comparison operator ($\bowtie$) is evaluated  using the values of
counters $a_{\phi,\psi}$ and $h_{\phi,\psi}$ at time instants 16 and 2
(enclosed in a circle in the figure), resulting in $\frac{8}{2}=4$.
When the same formula is evaluated at time instant 18, the portion of
the history trace considered contains both a left-open
$(\phi_{|2},\psi_{|5})$ pair and a right-open
$(\phi_{|17},\psi_{|19})$ one. The lhs of the comparison operator is
evaluated using the values of counters  $a_{\phi,\psi}$,
$b_{\phi,\psi}$, and $h_{\phi,\psi}$  at time instants 19 and 5
(enclosed in  a triangle in the figure ); its value is $\frac{5}{1}=5$.
Now consider the formula  $\mathfrak{D}_{\bowtie n}^{12}\{(\phi,
\psi)\}$. When evaluated at time instant 15, it has a left-open pair
$(\phi_{|2},\psi_{|5})$. The values of the counters $a_{\phi,\psi}$,
$b_{\phi,\psi}$, and $h_{\phi,\psi}$ consider to compute the lhs of
the comparison operator are those at time instants 16 and 4 (enclosed
in a square in the figure); the lhs evaluates to $\frac{5}{1}=5$. If
the same formula is evaluated at time instant 18, we find only a
right-open pair $(\phi_{|17},\psi_{|19})$. The lhs of the comparison
operator is evaluated using the value of counters $a_{\phi,\psi}$ and
$h_{\phi,\psi}$ considered at time instants 19 and 7 (enclosed in a
hexagon in the figure); its value is $\frac{5}{1}=5$.


\begin{figure*}
\centering
\input{figures/dmod}
\caption{Example of history trace for the $\mathfrak{D}$ modality}
\label{fig:dmod}
\end{figure*}    



%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "soca2014"
%%% End: 


==> plots/paramDn2mem.tex <==
\begin{tikzpicture}[scale=0.65]
    \begin{axis}[
      xlabel={$card(S)$},
      xlabel near ticks,
      ylabel={Memory (MB)},
      ylabel near ticks,
      legend pos=north west
    ]
\addplot[color=black, mark=diamond*] table [x="Parameter", y="Memory (MB)", col sep=comma] {../csvs/D-d-0-100-h-10.csv};
    \end{axis}
\end{tikzpicture}


==> plots/paramDn2time.tex <==
\begin{tikzpicture}[scale=0.65]
    \begin{axis}[
      legend pos=north west,
      xlabel={$card(S)$},
      xlabel near ticks,
      ylabel={Time (s)},
      ylabel near ticks
    ]
\addplot[color=lightgray,mark=*] table [x="Parameter", y="SMT time (s)", col sep=comma] {../csvs/D-d-0-100-h-10.csv};
\addplot[color=darkgray, mark=square*] table [x="Parameter", y="User time (s)", col sep=comma] {../csvs/D-d-0-100-h-10.csv};
\legend{SMT time, Total time}
    \end{axis}
\end{tikzpicture}


==> plots/sparseness-mem.tex <==

\begin{tikzpicture}[scale=0.65]
\begin{axis}[
		legend pos=north west,
		xlabel=Trace length,
		height=\plotHeight,
		width=\plotWidth,
		ylabel=Memory (B),
		ymax=200000000
		]

\addplot[color=lightgray, mark=square*] table [x="Parameter", y="Zot Memory (B)", col sep=comma] {plots/data-C-1.csv};
\addplot[color=lightgray, mark=square*] table [x="Parameter", y="Zot Memory (B)", col sep=comma] {plots/data-C-2.csv};
\addplot[color=lightgray, mark=square*] table [x="Parameter", y="Zot Memory (B)", col sep=comma] {plots/data-C-3.csv};
\addplot[color=lightgray, mark=square*] table [x="Parameter", y="Zot Memory (B)", col sep=comma] {plots/data-C-4.csv};
\addplot[color=lightgray, mark=square*] table [x="Parameter", y="Zot Memory (B)", col sep=comma] {plots/data-C-5.csv};
\addplot[color=lightgray, mark=square*] table [x="Parameter", y="Zot Memory (B)", col sep=comma] {plots/data-C-6.csv};
\addplot[color=lightgray, mark=square*] table [x="Parameter", y="Zot Memory (B)", col sep=comma] {plots/data-C-7.csv};
\addplot[color=black, mark=*] table [x="Parameter", y="Zot Memory (B)",  col sep=comma] {plots/data-B.csv};


\node at (axis cs:145,150000000) [anchor=north east] {100\%};
\node at (axis cs:240,150000000) [anchor=north east] {50\%};
\node at (axis cs:350,150000000) [anchor=north east] {33\%};
\node at (axis cs:460,150000000) [anchor=north east] {25\%};
\node at (axis cs:570,150000000) [anchor=north east] {20\%};
\node at (axis cs:640,110000000) [anchor=north east] {16.6\%};
\node at (axis cs:620,45000000) [anchor=north east] {14.3\%};


\legend{\qf,,,,,,,\ct}
\end{axis}
\end{tikzpicture}



